Entangled View-Epipolar Information Aggregation for Generalizable Neural Radiance Fields

Generalizable NeRF can directly synthesize novel views across new scenes, eliminating the need for scene-specific retraining in vanilla NeRF. A critical enabling factor in these approaches is the extraction of a generalizable 3D representation by aggregating source-view features. In this paper, we propose an Entangled View-Epipolar Information Aggregation method dubbed EVE-NeRF. Different from existing methods that consider cross-view and along-epipolar information independently, EVE-NeRF conducts the view-epipolar feature aggregation in an entangled manner by injecting the scene-invariant appearance continuity and geometry consistency priors to the aggregation process. Our approach effectively mitigates the potential lack of inherent geometric and appearance constraint resulting from one-dimensional interactions, thus further boosting the 3D representation generalizablity. EVE-NeRF attains state-of-the-art performance across various evaluation scenarios. Extensive experiments demonstate that, compared to prevailing single-dimensional aggregation, the entangled network excels in the accuracy of 3D scene geometry and appearance reconstruction. Our code is publicly available at https://github.com/tatakai1/EVENeRF.

==> figs/intro_fig1.tex <==
%  \begin{figure*}
%     \centering
%     \includegraphics[width=1.0\textwidth]{figs/intro4.png}
%     \caption{Considering that each sampling point along the target ray has a mapping relationship with sampling points on the epipolar lines in each known view as depth increases (a), existing approaches\cite{suhail2022generalizable}\cite{wang2021ibrnet}\cite{varma2022attention} employ self-attention to aggregate the features of correspondences between sampling points for cross-view aggregation and perform epipolar aggregation of sampling points along the epipolar lines within individual views (b). However, when aggregating solely cross-view information, the model suffers from artificial appearance  in rendering results due to the absence of the complete epipolar line information. Conversely, when aggregating only epipolar information, the model's ability to reason about geometry is constrained, leading to discontinuities in the depth map due to the lack of multi-views information. Our proposed Dual-NeRF effectively addresses above issues (c).}
%     \label{intro_fig1}
% \end{figure*}


%  \begin{figure*}[ht]
%     \centering
%     \begin{subfigure}{0.202\linewidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{figs/sub_intro1.png}
% 		\caption{Source views}
% 	\end{subfigure}
% \centering
%  \begin{subfigure}{0.366\linewidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{figs/sub_intro2.png}
% 		\caption{Two ways of generalizable information aggregation}
% 	\end{subfigure}
%  \centering
%  \begin{subfigure}{0.421\linewidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{figs/sub_intro3.png}
% 		\caption{Generalizable novel view synthesis}
%         \label{intro1_sub3}
% 	\end{subfigure}
%  \caption{Given the sampling points  along a target ray that are re-projected on the epipolar lines in each source view (a), existing approaches~\cite{suhail2022generalizable, varma2022attention} employ attention mechanism to aggregate the cross-view features for each sampling point and perform epipolar aggregation of sampling points along the epipolar lines within individual views (b), either sequentially or circularly. However, our investigation reveals the limitations in existing strategies: exclusively aggregating cross-view information results in rendering artifacts, stemming from the absence of \textbf{appearance continuity between adjacent depth} provided by epipolar cues. Conversely, relying solely on epipolar information leads to depth map discontinuities due to the absence of \textbf{geometry consistency across multiple views}. Our proposed EVE-NeRF harnesses both cross-view and along-epipolar information in an entangled manner and effectively addresses the above issues (c).}
% 	\label{intro_fig1}
% \end{figure*}

 \begin{center}
    \centering
    \captionsetup{type=figure}
		\includegraphics[width=0.20\linewidth]{figs/sub_intro1.png}
		\includegraphics[width=0.363\linewidth]{figs/sub_intro2.png}
		\includegraphics[width=0.417\linewidth]{figs/sub_intro3.png}
 \captionof{figure}{Given the sampling points  along a target ray that are re-projected on the epipolar lines in each source view, existing approaches~\cite{suhail2022generalizable, varma2022attention} employ attention mechanism to aggregate the cross-view features for each sampling point and perform epipolar aggregation of sampling points along the epipolar lines within individual views, either sequentially or circularly. However, our investigation reveals the limitations in existing strategies: exclusively aggregating cross-view information results in rendering artifacts, stemming from the absence of \textbf{appearance continuity between adjacent depth} provided by epipolar cues. Conversely, relying solely on epipolar information leads to depth map discontinuities due to the absence of \textbf{geometry consistency across multiple views}. Our proposed EVE-NeRF harnesses both cross-view and along-epipolar information in an entangled manner and effectively addresses the above issues.}
	\label{intro_fig1}
 \end{center}


==> template/finetune_blender.tex <==
\begin{table*}
\centering
% \resizebox{\columnwidth}{!}{
\begin{subtable}{1.\linewidth}
      \centering
        \begin{tabular}{cccccccccc}
            \toprule
            Models & Lego& Chair&  Drums & Ficus&  Hotdog&  Materials&  Mic&  Ship \\  
            \midrule
            LLFF~\cite{mildenhall2019local} & 24.54 &28.72 &21.13 &21.79& 31.41 &20.72& 27.48 &23.22 \\
            NeRF~\cite{mildenhall2021nerf}  &32.54 &33.00 &25.01 &30.13 &36.18 &29.62 &32.91 &28.65      \\
            MipNeRF~\cite{barron2021mip}  &35.70 &35.14 &25.48& 33.29 &37.48 &30.71 &36.51 &30.41 \\
            % NLF~\cite{suhail2022light} &35.76& 35.30& 25.83 &33.38& 38.66 &35.10 &35.32 &30.94 \\
             EVE-NeRF  &31.80      &33.63     &25.32          & 28.58       &37.49           &28.88       &33.12     & 28.90       \\
            \bottomrule
        \end{tabular}
        \caption{PSNR$\uparrow$}
    \end{subtable}%

\begin{subtable}{1.\linewidth}
      \centering
        \begin{tabular}{cccccccccc}
            \toprule
            Models & Lego& Chair&  Drums & Ficus&  Hotdog&  Materials&  Mic&  Ship \\  
            \midrule
            LLFF~\cite{mildenhall2019local} &0.911 &0.948 &0.890 &0.896 &0.965 &0.890 &0.964 &0.823 \\
            NeRF~\cite{mildenhall2021nerf} &0.961 &0.967 &0.925& 0.964& 0.974 &0.949& 0.980 &0.856 \\
            MipNeRF~\cite{barron2021mip} &0.978& 0.981 &0.932 &0.980 &0.982& 0.959 &0.991 &0.882 \\
            % NLF~\cite{suhail2022light}& 0.978 &0.981& 0.932& 0.980 &0.982& 0.959 &0.991& 0.882\\
             % GNT  & 0.963     &0.846     &  0.852        &  0.934      &   0.752        & 0.893      &  0.936   &  0.935      \\
             EVE-NeRF  &0.976      &0.985     &0.948          & 0.966       & 0.990        &0.966       &0.986     &  0.934      \\
            \bottomrule
        \end{tabular}
        \caption{SSIM$\uparrow$}
    \end{subtable}%

\begin{subtable}{1.\linewidth}
      \centering
        \begin{tabular}{cccccccccc}
            \toprule
            Models & Lego& Chair&  Drums & Ficus&  Hotdog&  Materials&  Mic&  Ship \\   
            \midrule
            LLFF~\cite{mildenhall2019local} &0.110 &0.064 &0.126 &0.130 &0.061 &0.117 &0.084 &0.218 \\
            NeRF~\cite{mildenhall2021nerf} &0.050& 0.046& 0.091& 0.044& 0.121& 0.063 &0.028& 0.206 \\
            MipNeRF~\cite{barron2021mip} &0.021& 0.021& 0.065& 0.020 &0.027 &0.040 &0.009& 0.138 \\
            % NLF~\cite{suhail2022light}& 0.010& 0.012& 0.045& 0.010 &0.009& 0.011& 0.008& 0.084 \\
             % GNT  & 0.060     &0.116     & 0.109         &  0.061      &  0.153         &  0.092     &  0.080   & 0.076       \\
             EVE-NeRF  & 0.035      &0.023     &0.063          & 0.041       & 0.024         & 0.046      &0.014    & 0.134      \\
            \bottomrule
        \end{tabular}
        \caption{LPIPS$\downarrow$}
    \end{subtable}%
% \begin{tabular}{cccccccccc}
% \toprule 
% Models & Room& Fern&  Leaves & Fortress&  Orchids&  Flower&  T-Rex&  Horns \\  
% & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
% \midrule
% PixelNeRF & 18.66 & 0.588 & 0.463  &22.65 &0.808 &0.202 &- &- &-\\
% IBRNet & 25.17 & 0.813 & 0.200  &26.73 &0.908 &0.101 &23.60  &0.785  &0.180 \\
% GPNR & 25.35 & 0.818 & 0.198  &\textbf{28.29} &0.927 &0.080 &25.72  &0.880  &0.175 \\
% NeuRay & 25.72 & 0.880 & 0.175  &26.48 &0.944 &0.091 &24.12  &0.860  &0.170 \\
% GNT & 18.66 & 0.588 & 0.463  &26.48 &0.944 &0.091 &27.19  &0.912  &0.083 \\
% Dual-NeRF & \textbf{27.16} & \textbf{0.912} & \textbf{0.134}  &27.03 &\textbf{0.952} &\textbf{0.072} &\textbf{28.01}  &\textbf{0.935}  &\textbf{0.083}\\
% \bottomrule
% \end{tabular}

% }
\caption{ Single-scene fine-tuned comparison results for Blender dataset
}
\vspace{-0.05in}
\label{tab:finetune_blender}
\end{table*}



% LLFF数据集单场景finetune对比结果

==> template/fps_compare.tex <==
\begin{table}[t]
\centering
% \resizebox{\columnwidth}{!}{

\begin{tabular}{lccc}
\toprule 
Model & Storage (MB) & Rendering Time (s) & PSNR$\uparrow$ \\           
\midrule
GNT~\cite{varma2022attention} & 112 & 208 & 24.55 \\
EVE-NeRF & 53.8 & 194 & 26.07 \\
\bottomrule
\end{tabular}

% }
\caption{
Efficiency comparison results.
% The results demonstrate that both the along-epipolar perception and the muti-view calibration effectively enhance the aggregation capability of a single dimension. Moreover, compared to other dual-branch structures, EVE-NeRF exhibits superior generalization performance.
}
\vspace{-0.05in}
\label{tab:fps_compare}
\end{table}


% Ablation study 采用低分辨率的setting 1进行训练并在分辨率为$504 \times 378$的LLFF中测试。结果显示view-independence geometry prior和muti-view weights regressor 可以有效提升单个维度聚合的能力。另外，相比其他双分支结构，Dual-NeRF具有更好的generalization performance。

